Self-Stabilizing Snapshot Objects for Asynchronous Fail-Prone Network Systems

A snapshot object simulates the behavior of an array of single-writer/multi-reader shared registers that can be read atomically. Delporte-Gallet et al. proposed two fault-tolerant algorithms for snapshot objects in asynchronous crash-prone message-passing systems. Their first algorithm is \emph{non-blocking}; it allows snapshot operations to terminate once all write operations have ceased. It uses $O(n)$ messages of $O(n \nu)$ bits, where $n$ is the number of nodes and $\nu$ is the number of bits it takes to represent the object. Their second algorithm allows snapshot operations to always terminate independently of write operations. It incurs $O(n^2)$ messages. The fault model of Delporte-Gallet et al. considers node crashes. We aim at the design of even more robust snapshot objects via the lenses of self-stabilization---a very strong notion of fault-tolerance. In addition to Delporte-Gallet et al.'s fault model, our self-stabilizing algorithm can recover after the occurrence of transient faults; these faults represent arbitrary violations of the assumptions according to which the system was designed to operate. We propose self-stabilizing variations of Delporte-Gallet et al.'s non-blocking algorithm and always-terminating algorithm. Our algorithms have similar communication costs to the ones by Delporte-Gallet et al. and $O(1)$ recovery time from transient faults. The main differences are that our proposal considers repeated gossiping of $O(\nu)$ bit messages and deals with bounded space. We also consider an input parameter, $\delta$, for which we claim an ability to balance the costs of snapshot operations. We validate our correctness proof, evaluate the performance of Delporte-Gallet et al.'s algorithms and our proposed variations and investigate the properties of $\delta$ via PlanetLab experiments, where significant latency and communication costs reduction are observed.

==> snapshotEvaluation/oldEvalSection.tex <==
\remove{

\subsection{Results}

In this section we use lemmas \ref{thm:latencyBounds} and \ref{thm:communicationCostsBounds} to anticipate the results of the experiments, we present the real results of the experiments and then compare the expectations with the real results. Based on the values of table \ref{tab:delays}, we can calculate what value the variables from definition \ref{def:latencyDefinition} will have in these experiments, namely that $\mu_1 = \mu_2 = \lambda = 3$.

\subsubsection*{Experiment 1: Scalability of write operations with respect to write operations}
\label{sec:exp1}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp1_all.pdf}
    \captionof{figure}{The result of experiment 1, showing the write latency of all algorithms.\newline}
    \label{fig:exp1_all}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp1_1_and_3.pdf}
    \centering
    \captionof{figure}{The result of experiment 1, showing the write latency of algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}.}
    \label{fig:exp1_1_and_3}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp1_2_and_4.pdf}
    \centering
    \captionof{figure}{Experiment~1's results for the write latency of algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}.}
    \label{fig:exp1_2_and_4}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp1m_all.pdf}
    \centering
    \captionof{figure}{Experiment~1's results for number of quorum accesses per write operation of all algorithms. \EMS{OL, I think that it shows only algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}}}
    \label{fig:exp1m_all}
\end{minipage}
\end{figure}

Figure \ref{fig:exp1_all} shows the result of Experiment 1 for all of the studied algorithms. We can see that with the experiment setup presented in Table~\ref{tab:delays}, algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} are $\lambda/\kappa$ times faster at writing than algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}, but that the write latency of all of them does not depend on the number of writers. Recall that this Experiment 1 is a control experiment, which aims not at bringing novel research insights.

We begin by considering algorithms~\ref{alg:0disCongif} and~\ref{alg:9disCongif}. From Lemma~\ref{thm:latencyBounds}, we anticipate that the write latency will be $\kappa$ (no matter the number of writers). In Figure~\ref{fig:exp1_1_and_3}, we observe that the write latency is slightly longer than $\kappa$ and that it increases with the number of writers. This can be explained by Remark~\ref{thm:planetLab} since increasing the number of writers implies a higher load on the nodes. We also observe in Figure~\ref{fig:exp1_1_and_3} that the overhead difference between algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} is negligible. From Lemma~\ref{thm:communicationCostsBounds} we anticipate that one quorum access will be used per write operation. Figure~\ref{fig:exp1m_all} validates this anticipation.

Next, we consider algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}. From Lemma~\ref{thm:latencyBounds}, we know that the lower bound on the write latency is $\mu_1 = \lambda$ for both of algorithms. This lower bound should be possible to match since Experiment 1 does not consider the execution of snapshot operations. In Figure~\ref{fig:exp1_2_and_4}, we observe that the write latency matches $\mu_1 = \lambda$. By the pseudo-code in algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} (for all values of $\delta$), we see that these algorithms should have similar latencies that independent of the number of writers. Moreover, since snapshot operations are absent from Experiment~1, the $\delta$-parameter should not play a role. The greatest difference between any two measured latencies of algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} is 20 milliseconds, \ie less than $1\%$ of the latency, thus we consider this to be insignificant. From Lemma~\ref{thm:communicationCostsBounds}, we predicts one quorum access per write operation. Figure \ref{fig:exp1m_all} validates this prediction.


\remove{

\OL{Below begins the old text, before I grouped anticipation and result, per algo, together. I think the new style works better. What do you think?}


From Lemma~\ref{thm:latencyBounds} we anticipate that the write latency is $\kappa$ for algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}, and $\mu$ for algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}. These lower bounds should be possible to matched since Experiment 1 does not consider the execution of snapshot operations. From Lemma~\ref{thm:communicationCostsBounds} we anticipate that exactly one quorum accesses is needed per write operation for all algorithms. We also remind the reader that this experiment is only a control experiment, which brings no novel research insights.

The result of Experiment~1 is shown in figures~\ref{fig:exp1_all} to~\ref{fig:exp1m_all}. From Figure~\ref{fig:exp1_all} we see that the write latency of all algorithms matches Lemma~\ref{thm:latencyBounds}. That is, for algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}, just a single quorum access is needed, which takes $\kappa$ seconds (see Table~\ref{tab:delays}). For algorithms \ref{alg:9disCongif} and \ref{alg:terminating}, a write operation is only handled once per do-forever iteration, \ie once every $\lambda$ seconds. Figure~\ref{fig:exp1_1_and_3} takes a closer look on the result for algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}. We see that there is a small increase in write latency as the number of writers increases, which is anticipated since it means a higher load on the nodes. But still, this overhead difference between algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} is negligible. Figure~\ref{fig:exp1_2_and_4} takes a closer look on the result for algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}. We see that algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} (for all values of $\delta$) have similar latencies that are also independent of the number of writers. Since there are only writers, and no snapshotters, the $\delta$-parameter should not play a role. The greatest difference between any two results is 20 milliseconds, \ie less than $1\%$ of the latency, thus it is insignificant. We now turn to  take a look at Figure~\ref{fig:exp1m_all}, where we see that the number of quorum accesses of all algorithms is one, which fits with Lemma~\ref{thm:communicationCostsBounds}.

%\OL{I think the remaining text below can be removed. I have integrated it into the previous two paragraphs}




\EMS{OL, for every such subsubsection, please first state what are the anticipated results --- try to cite lemmas 6.1 and 6.2 when possible. Then say what was observed. If there is a difference between what was anticipated and what was observed, please try to explain why --- hopefully lemmas 6.1 and 6.2 explains it all. --- also, for this particular experiment, please remind the reader that experiment 1 is a control experiment --- no real new discoveries. }
The result of experiment 1 is shown in figures~\ref{fig:exp1_all} to~\ref{fig:exp1m_all}. From Figure~\ref{fig:exp1_all} we see that the write latency, for all algorithms, appears to be unaffected by the number of writers. A 1 second latency is expected from algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}, since the write operation just needs a single quorum access, which take \EMS{OL, please put the Greek letter here for the quorum delay an refer to Table 1}. In algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}, a write operation can only be handled every 3 seconds, which is the do-forever delay \EMS{OL, please put the Greek letter here for the quorum delay an refer to Table 1}. Because this experiment assumes the absence of snapshot operations, and thus there is never any need to invoke, and wait for, $\mathrm{baseSnapshot}()$. The write latency we expect is therefore \EMS{OL, please put the Greek letter here for the quorum delay an refer to Table 1} 3 seconds, which is also what we observe. Figure~\ref{fig:exp1_1_and_3} takes a closer look of the write latency of algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}. We can see a small increase in write latency as the number of writers increases, but that is not a contradiction to the previous observations, since more write operations must mean a higher load on the nodes. It is also clear that the overhead difference between algorithms~\ref{alg:disCongif} and~\ref{alg:0disCongif} is negligible. The write latency of algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} is shown in Figure~\ref{fig:exp1_2_and_4}. We see that algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} (for all values of $\delta$) have similar latencies that are also independent of the number of writers. Since there are only writers, and no snapshotters, the $\delta$-parameter should play no role. The greatest difference between any two results is 20 milliseconds, \ie less than $1\%$ of the latency, thus it is insignificant. 
%
%If there truly was a difference between how Algorithm~\ref{alg:terminating} behaves for different number of writers and different values of $\delta$ in this experiment, the difference would have been larger. 
%
We now turn to look at Figure~\ref{fig:exp1m_all}, which shows the number of write quorum accesses per write operation for all algorithms. As expected \EMS{OL, please cite the relevant lemma}, only a single quorum access is needed for all algorithms, since the $\sWrite()$/$\mathrm{baseWrite}()$ functions behave in identical ways and do not depend on the number of writers.

}

\subsubsection*{Experiment 2: Scalability of write operations with respect to snapshot operations}
\label{sec:exp2}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp2_all.pdf}
    \captionof{figure}{The result of experiment 2, showing the write latency of all algorithms.\newline}
    \label{fig:exp2_all}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp2_1_and_3.pdf}
    \centering
    \captionof{figure}{The result of experiment 2, showing the write latency of  algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}.}
    \label{fig:exp2_1_and_3}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp2_all_only_mixed.pdf}
    \captionof{figure}{The result of experiment 2, showing the write latency of all algorithms but only for mixed writers/snapshotters. Note that when $\delta = 1,000,000$ and there was only one snapshotter, its snapshotting was entirely starved in some runs, and just slow in other runs.}
    \label{fig:exp2_all_only_mixed}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp2_all_only_pure_writers.pdf}
    \centering
    \captionof{figure}{The result of experiment 2, showing the write latency of all algorithms but only for pure writers. Note that when there are 15 snapshotters, there are no pure writers.}
    \label{fig:exp2all_only_pure_writers}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp2_2_and_4.pdf}
    \caption{The result of experiment 2, showing the write latency of algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} for $\delta \in \{0, 5, 20 \}$.}
    \label{fig:exp2_2_and_4}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp2m_all.pdf}
    \centering
    \captionof{figure}{The result of experiment 2, showing the number of write-quorum accesses per write operation of all algorithms.}
    \label{fig:exp2m_all}
\end{minipage}
\end{figure}

Figure \ref{fig:exp2_all} shows the result of Experiment 2 for all algorithms. With the exception of a single peak (for Algorithm~\ref{alg:terminating} at 5 snapshotters), we see that the write latency does not change when the number of snapshotters increases and that algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} are $\lambda/\kappa$ times faster at writing than algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}.

We begin by considering algorithms \ref{alg:0disCongif} and \ref{alg:disCongif}. Based on Lemma~\ref{thm:latencyBounds}, we anticipate that the write latency will be $\kappa$ seconds, no matter the number of snapshotters. In Figure~\ref{fig:exp2_1_and_3}, we see that the write latency is slightly longer than $\kappa$ and that it increases with the number of writers. This can be explained by Remark~\ref{thm:planetLab} since increasing the number of writers implies a higher load on the nodes. We also observe that the overhead Algorithm~\ref{alg:disCongif} brings compared to Algorithm~\ref{alg:0disCongif} is negligible. Lemma~\ref{thm:communicationCostsBounds} predicts one quorum access per write operation and Figure~\ref{fig:exp2m_all} validates this prediction.

Next, we consider algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}. By Lemma~\ref{thm:latencyBounds}, we know $\lambda$ is the lower bound on the write latency. With the $\zeta$ delay between client write operations and Corollary \ref{thm:synchronizationBehavior} in mind, we proceed to look at the results in figures~\ref{fig:exp2_all} and~\ref{fig:exp2_2_and_4}. \EMS{OL, what about Figure 11? If you refer to it only later then it should appear later.} \OL{fig 11 is refered to (before fig 12) in the beginning of the previous paragraph} From these figures we observe that the write latency is actually quite close to the lower bound of Lemma~\ref{thm:latencyBounds} in most cases, despite concurrent snapshot operations taking time in the do-forever loop. This is explained by the $\zeta$ delay that prevents the system from being saturated with write operations. For Algorithm \ref{alg:terminating} with $\delta = 1,000,000$, we see a peak at 5 writers. With 5 writers and a large $\delta$, the snapshot latency is potentially long, which we know from Corollary \ref{thm:synchronizationBehavior} will lead to a long write latency as well. For higher values of $\delta$, the snapshot latency will be lower and for more snapshotters, we know from Corolloary \ref{thm:synchronizationBehavior} that it will be easier for all nodes to complete their snapshot operations, which means the peak is just a peak, and not wider. \EMS{OL, this is not an explanation. The reader might think that we might have a bug there or an experiment outlier. To me it seems that we need more experiments with more numbers of writers, like 3, 4, 6, 7 and more $\delta$s like 10, 15, 50 and 200. I think that there might be a pattern emerging where the trade off between write and snapshot latencies have a sweet spot. What do you think?} \OL{But what do we write here then to explain the peak? I think we should avoid the synchronization behavior in the future experiments 1-4 because it obscures the effect of $\delta$, and then we can have a separate experiment where we explore the synchronization.} From Figure~\ref{fig:exp2_2_and_4}, we see how Algorithm \ref{alg:9disCongif} is somewhat slower than Algorithm \ref{alg:terminating}. The reason could be that the flooding mechanism used for the reliable broadcast requires a large amount of locking. For each message receieved, the lock belonging to the set of received messages needs to be acquired. Due to the flooding mechanism, a single message sent using the reliable broadcast function will be received many times by each node, potentially $O(n^2)$ times. This locking takes time and reduces possible concurrency between threads. Lemma~\ref{thm:communicationCostsBounds} predicts one quorum access per write operation. Figure~\ref{fig:exp2m_all} validates this prediction.

\remove{

\OL{Old style is below.}





From lemma \ref{thm:latencyBounds} we expect the write latency to be $\kappa$ seconds for algorithms \ref{alg:0disCongif} and \ref{alg:disCongif}, and at least $\mu$ for algorithms \ref{alg:9disCongif} and \ref{alg:terminating}. Unlike experiment 1, the write latency might be longer than the lower bound due to concurrent snapshots. From lemma \ref{thm:communicationCostsBounds} we expect that exactly one quorum accesses is needed per write operation for all algorithms.

The result of experiment 2 is shown in figures~\ref{fig:exp2_all} to~\ref{fig:exp2m_all}. From figure~\ref{fig:exp2_all} we see that the write latency of all algorithms, except Algorithm~\ref{alg:terminating} for $\delta = 1,000,000$, matches (the lower bounds of) lemma \ref{thm:latencyBounds} closely. We see a much longer write latency for Algorithm~\ref{alg:terminating} when $\delta = 1,000,000$ and the number of snapshotters is 5. The reason for this is a synchronization behavior that emerges on algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating} when a node is a writer and a snapshotter. If a node invokes baseSnaphot() in its do-forever loop, the node cannot complete another write until baseSnapshot() returns. This means that if the snapshot latency is long, so will the write latency be. When $\delta = 1,000,000$, nodes will never block their write operations in order to help another node, which means that in the case of this experiment, the snapshot latency can be quite long. The result of the synchronization behavior is most clearly shown when there are 5 snapshotters. To understand this, we need to consider the synchronization behavior from the snapshotters' perspective.

A node that is writing and snapshotting will alternate between invoking baseWrite() and baseSnapshot() in the do-forever loop. When a node invokes baseSnapshot(), it will no longer write, and it will not start writing again until baseSnapshot() returns. As more and more nodes go from writing to snapshotting, there will be fewer and fewer writers, meaning that there will be less interruptions and all nodes' snapshot operations are more likely to complete. The effect is that the more of the writing nodes that are also snapshotting, the lower the snapshot latency can be. From the previous paragraph we also know that a lower snapshot latency means a lower write latency, which explains why the write latency peak is at 5 snapshotters. For lower values of $\delta$, the synchronization behavior is not needed to keep the snapshot latency low, since in that case writers will stop writing and help other nodes' snapshot anyway. This explains why the peak is only shown for $\delta = 1,000,000$.

In figure~\ref{fig:exp2_1_and_3}, it is shown how the write latency only has a small increase when the number of snapshotters increases for algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}. The reason is once again that more snapshotters must mean a higher load on the nodes. And just like experiment 1, the overhead of Algorithm \ref{alg:disCongif} compared to Algorithm \ref{alg:0disCongif} is very small.

A close-up of the result for algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}, $\delta \in \{0,5,20\}$, is shown in figure~\ref{fig:exp2_2_and_4}. We see that there is a slight increase in write latency as the number of snapshotters increases, which again is due to a higher load on the nodes. We also see that higher values of $\delta$ give a slightly longer write latency, which is due to the previously mentioned synchronization behavior. From this close-up we even see a peak for $\delta = 20$ for 5 snapshotters, just like we saw a peak for $\delta = 1,000,000$ for 5 snapshotters in figure \ref{fig:exp2_all}. We finally see that Algorithm~\ref{alg:9disCongif} is slightly slower than Algorithm~\ref{alg:terminating}. The reason for this could be the reliable broadcast in combination with the locking. When flooding messages, variables need to be locked each time a message is received, and a single message broadcast will be received many times. Not only does the locking itself consume time, but all received messages must be handled one at a time and when they are being handled, they hold locks, which reduces the concurrency possible in other parts of the program as well.

We finally take a look at figure \ref{fig:exp1m_all}, where we see that the number of quorum accesses of all algorithms is one, which matches lemma \ref{thm:communicationCostsBounds}.

} %remove

\subsubsection*{Experiment 3: Scalability of snapshot operations with respect to snapshot operations}
\label{sec:exp3}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp3_all.pdf}
    \captionof{figure}{The result of experiment 3, showing the snapshot latency of all algorithms.}
    \label{fig:exp3_all}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp3_all_but_2.pdf}
    \centering
    \captionof{figure}{The result of experiment 3, showing the snapshot latency of algorithms~\ref{alg:0disCongif},~\ref{alg:disCongif} and~\ref{alg:terminating}.}
    \label{fig:exp3_all_but_2}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp3_1_and_3.pdf}
    \caption{The result of experiment 3, showing the snapshot latency of algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}.}
    \label{fig:exp3_1_and_3}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp3_4.pdf}
    \caption{The result of experiment 3, showing the snapshot latency of Algorithm~\ref{alg:terminating}.}
    \label{fig:exp3_4}
\end{minipage}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{snapshotEvaluation/exp3m_all.pdf}
    \captionsetup{justification=centering,margin=2cm}
    \caption{The result of experiment 3, showing the number of snapshot-quorum accesses and reliable broadcasts per snapshot operation of all algorithms.}
    \label{fig:exp3m_all}
\end{figure}

Figure \ref{fig:exp3_all} shows the snapshot latency of all algorithms for Experiment 3. We can see that the snapshot operations are completed in constant time for algorithms \ref{alg:0disCongif}, \ref{alg:disCongif} and \ref{alg:terminating} while they are completed in linear time for Algorithm \ref{alg:9disCongif}.

We begin by considering algorithms \ref{alg:0disCongif} and \ref{alg:disCongif}. Based on Lemma~\ref{thm:latencyBounds}, we anticipate that the snapshot latency will be $\kappa$ seconds, which is the lower bound. This lower bound should be matched since Experiment 3 does not consider the execution of write operations. In Figure~\ref{fig:exp3_1_and_3}, we observe that the snapshot latency is slightly longer than $\kappa = 1$ second and that it increases with the number of snapshotters. This can be explained by Remark~\ref{thm:planetLab} since increasing the number of snapshotters implies a higher load on the nodes. We also see that the overhead Algorithm \ref{alg:disCongif} brings compared to Algorithm \ref{alg:0disCongif} is negligible. From Lemma~\ref{thm:communicationCostsBounds}, we know that the lower bound on the number of quorum accesses per snapshot operation is one. Since there are no writers in Experiment 3, this lower bound should be matched, which Figure~\ref{fig:exp3m_all} validates.

Next, we consider Algorithm~\ref{alg:9disCongif}. Lemma~\ref{thm:latencyBounds} states that $\mu_1 = \lambda$ is the lower bound on the snapshot latency for Algorithm \ref{alg:9disCongif}. This should be possible to match for a single snapshotter, but not when there are multiple snapshotters. Figure \ref{fig:exp3_all} shows this is the case in practice. The snapshot latency grows linearly with the number of snapshotters since all nodes must handle every node's snapshot operation, and only one snapshot operation is handled at a time. Figure \ref{fig:exp3m_all} shows the number of quorum accesses per snapshot operation used. The reason more than one quorum access is used per snapshot operation is that a node may perform snapshot tasks on behalf of any node, meaning that a single snapshot operation is performed by multiple nodes, which will lead to more than one quorum access per operation. From figure \ref{fig:exp3m_all}, we see that the number of reliable broadcasts is always one more than the number of quorum accesses. The reason is that each quorum access will be successful (no interruptions by writers) and will be followed by a reliable broadcast of END (line \ref{ln:prevReg}). But for each snapshot operation, SNAP is also reliably broadcast (line \ref{ln:reliableBroadcastout}). These results lie within the bounds stated by Lemma \ref{thm:communicationCostsBounds}, but we also saw that they are not that close to the lower bounds.

We finally consider Algorithm \ref{alg:terminating}. Lemma \ref{thm:latencyBounds} states that $\mu_2 = \lambda$ is the lower bound on the snapshot latency for Algorithm \ref{alg:terminating}. This should be possible to match since there are no writers. Figure \ref{fig:exp3_4} shows this is the case in practice. Note that unlike Algorithm \ref{alg:9disCongif}, Algorithm \ref{alg:terminating} handles multiple snapshots at a time, which makes the lower bound possible to achieve for more than one snapshotter as well. Since there are only snapshotters, and no writers, the $\delta$-parameter should play no role. The greatest difference between any two results is 10 milliseconds, \ie less than $1\%$ of the latency, thus it is insignificant. Lemma \ref{thm:communicationCostsBounds} states that the lower bound on the number of quorum accesses per snapshot operation is two. Since there are no writers in Experiment 3, this lower bound should be possible to match. Figure \ref{fig:exp3m_all} shows this is the case in practice except for $\delta = 0$. The reason for this is similar to that of the case of Algorithm \ref{alg:9disCongif}, namely that more than one node may perform a single snapshot task. This only happens when $\delta = 0$, since for $\delta > 0$, a snapshot must have been concurrent with write operations before other nodes will help. As the number of snapshotters increases, the effect of this gets lower since if a node invokes $\mathrm{baseSnapshot}()$ for some other node's task, it would have invoked $\mathrm{baseSnapshot}()$ for its own task anyway.



\remove{



\OL{The old style of anticipation/result is below}

 

From lemma \ref{thm:latencyBounds} we expect the snapshot latency to be $\kappa$ for algorithms \ref{alg:0disCongif} and \ref{alg:disCongif}, which is the lower bound. This should be possible to achieve since no writers is the best-case scenario for algorithms \ref{alg:0disCongif} and \ref{alg:9disCongif}. We expect the snapshot latency of Algorithm \ref{alg:9disCongif} to be $\mu_1$ when there is one snapshotter, but larger for more snapshotters, since more than one snapshotter is not the best-case scenario for Algorithm \ref{alg:9disCongif}. We expect the snapshot latency of Algorithm \ref{alg:terminating} to be the lower bound $\mu_2$ for all number of snapshotters though, since Algorithm \ref{alg:terminating} should behave the same no matter the number of snapshotters. We note that given the values of table \ref{tab:delays}, $\mu_1 = \mu_2$ in this case. From lemma \ref{thm:communicationCostsBounds} we expect the number of quorum accesses to be one for algorithms \ref{alg:0disCongif}, \ref{alg:9disCongif} and \ref{alg:disCongif}, and two for Algorithm \ref{alg:terminating}, which are the lower bounds of the lemma, since experiment 3 should be the best-case scenario. Similarily, we expect the number of reliable broadcast operations to be two for Algorithm \ref{alg:9disCongif}.

The result of experiment 3 is shown in figures~\ref{fig:exp3_all} to~\ref{fig:exp3m_all}. From figure~\ref{fig:exp3_all} we see that the result matches the expectations we previosuly made, based on lemma \ref{thm:latencyBounds}. The reason for the linear increase in snapshot latency for Algorithm \ref{alg:9disCongif} is that Algorithm~\ref{alg:9disCongif} only handles one snapshot task at a time, while Algorithm~\ref{alg:terminating} handles several and that in algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}, snapshot operations are independent of each other. Figure~\ref{fig:exp3_all_but_2} shows the result for just algorithms~\ref{alg:0disCongif},~\ref{alg:disCongif} and~\ref{alg:terminating} where we more clearly see that the result matches lemma \ref{thm:latencyBounds} closely. By taking a closer look of the result for algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} in figure~\ref{fig:exp3_1_and_3}, we can see that their snapshot latencies are almost identical. This tells us that the overhead Algorithm~\ref{alg:disCongif} brings compared to Algorithm~\ref{alg:0disCongif} is very small. Just like in experiments 1 and 2, the operation latency is not entirely independent of the number of snapshotters, but that is expected since more snapshotters means a higher load on the nodes. In figure~\ref{fig:exp3_4}, only Algorithm~\ref{alg:terminating} is shown. Since there are only snapshotters, and no writers, the $\delta$-parameter should play no role. The greatest difference between any two results is 10 milliseconds, \ie less than $1\%$ of the latency, thus it is insignificant. 

Finally we take a look at the number of quorum accesses (related to snapshots) and reliable broadcast operations that are needed per snapshot operation in figure~\ref{fig:exp3m_all}. We see that algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} use one quorum access per snapshot operation. This is expected since there are no writers that can interrupt them. We see that Algorithm~\ref{alg:terminating} for $\delta \neq 0$ uses two quorum accesses. This is also excpected: one for the snapshot and one for $\sStore()$. For the case of $\delta = 0$, we see that a lower number of snapshotters means more quorum accesses per snapshot operation, which does not match our initial expectations. The reason is that when $\delta = 0$, other nodes can also perform the lone snapshotter's task. Sometimes the broadcast in line~\ref{ln:ssnPlusOne2} happens with such a timing that other nodes will start that task before the result from $\sStore()$ arrives to them. As the number of snapshotters increases, the effect of this gets lower since if a node invokes $\mathrm{baseSnapshot}()$ for some other node's task, it would have invoked $\mathrm{baseSnapshot}()$ for its own task anyway. Figure~\ref{fig:exp3m_all} also shows that Algorithm~\ref{alg:9disCongif} uses more than one quorum access per snapshot operation even though it might appear from the pseudocode that only one is needed. The cause of this is similar to that of Algorithm~\ref{alg:terminating}, namely that more than one node will $\mathrm{baseSnapshot}()$ for each client-side snapshot operation. The dashed line shows the number of reliable broadcast operations Algorithm~\ref{alg:9disCongif} performes per snapshot operation. It is always one more than the number of quorum accesses, the reason being that an $\mathrm{END}$ message is reliably broadcast for each quorum access (which will always succeed on the first attempt) and one $\mathrm{SNAP}$ message is reliably broadcast in the beginning of $\sSnapshot()$.

} % remove

\subsubsection*{Experiment 4: Scalability of snapshot operations with respect to write operations}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp4_all.pdf}
    \captionof{figure}{The result of experiment 4, the snapshot latency of all algorithms.\newline}
    \label{fig:exp4_all}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp4_4.pdf}
    \centering
    \captionof{figure}{The result of experiment 4, showing the snapshot latency of Algorithm~\ref{alg:terminating}.}
    \label{fig:exp4_4}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp4_all_only_mixed.pdf}
    \captionof{figure}{The result of experiment 4, showing the snapshot latency of all algorithms but only mixed writers/snapshotters.}
    \label{fig:exp4_all_only_mixed}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp4_all_only_pure_snapshotters.pdf}
    \centering
    \captionof{figure}{The result of experiment 4, showing the snapshot latency of all algorithms but only for pure snapshotters. Note that at 15 writers, there are no pure snapshotters.}
    \label{fig:exp4_all_only_pure_snapshotters}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp4m_all.pdf}
    \captionof{figure}{The result of experiment 4, showing the number of snapshot-quorum accesses and reliable broadcasts per snapshot operation of all algorithms.}
    \label{fig:exp4m_all}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp4m_4.pdf}
    \centering
    \captionof{figure}{The result of experiment 4, showing the number of snapshot-quorum accesses per snapshot operation of Algorithm~\ref{alg:terminating}.}
    \label{fig:exp4m_4}
\end{minipage}
\end{figure}

Figure \ref{fig:exp4_all} shows the snapshot latency of all algorithms for Experiment 4. We see that for algorithms \ref{alg:0disCongif} and \ref{alg:disCongif}, the snapshot latency grows unbounded as the number of writers increases, while the snapshot latency remains bounded for algorithms \ref{alg:9disCongif} and \ref{alg:terminating}.

We begin by considering algorithms \ref{alg:0disCongif} and \ref{alg:disCongif}. The snapshot latency of them is shown in figure \ref{fig:exp4_all}. We see that the latency is low when there is just one writer, but that the latency grows unbounded as the number of writers increases. This is due to the writers interrupting the snapshotters all the time and illustrates that algorithms \ref{alg:0disCongif} and \ref{alg:disCongif} indeed allow starvation of snapshotters. The result matches lemma \ref{thm:latencyBounds}, which states the the lower bound on the latency is $\kappa$, but that there is no upper bound. In figure we see the number of quorum accesses used. Just like the latency, it starts low but grows unbounded, also matching Lemma \ref{thm:communicationCostsBounds}.

Next up we consider Algorithm \ref{alg:9disCongif}, whose latency is shown in figure \ref{fig:exp4_all}. We see that the latency is significantly longer than Algorithm \ref{alg:terminating}. We know the reason from Experiment 3, namely that many snapshotters lead to a long snapshot latency. We also see an increase when the number of writers increases, which is due to more interruptions and work in the do-forever loop. All in all the latency is much longer than the lower bound stated by Lemma \ref{thm:latencyBounds}. In figure \ref{fig:exp4m_all} we see that the number of quorum accesses starts close the the lower bound, but increases when the number of writers increases, which is because they are interrupted more often. When the snapshots are interrupted more often, it takes a longer time to complete them, and more nodes get the chance to try to complete them, which will increase the number of reliable broadcasts of END. But the number of reliable broadcasts does not increase as fast as the number of quorum accesses, since there will be one extra reliable broadcast for each new node helping, but one extra quorum access for every interruption. The latter are more numerous.

Finally we consider Algorithm \ref{alg:terminating}. Lemma \ref{thm:latencyBounds} states that the lower bound on the snapshot latency is $\mu_2 = \lambda$. Since there are concurrent writes, we anticipate the actual latency will be higher than this, but that the latency will be close to $\lambda$ when there is just one writer. In figure \ref{fig:exp4_4} we see that with one writer, the snapshot latency is slightly longer than 3 seconds when $\delta = 0$ and slightly longer than 4 seconds when $\delta \neq 0$. That $\delta = 0$ gives the lowest snapshot latency is expected, since it allows no concurrent write operations before all nodes will help with the snapshot operation. We also see that as the number of writers increases, so does the snapshot latency. What may seem surprising is how similar the latencies are for different values of $\delta$, especially for higher number of writers, and that snapshotters are not starved for $\delta = 1,000,000$. This is due to the synchronization effect described in section~\ref{sec:exp2}, which makes sure that snapshot operations cannot starve even when $\delta = \infty$. When it comes to the number of quorum accesses, lemma \ref{thm:communicationCostsBounds} states that two is the lower bound. We anticipate that for one writer, the number of quorum accesses will be close to two (since there will be few interruptions), and that the number of quorum accesses will increase as the number of writers increases. In figure \ref{fig:exp4m_4} we see that the result mostly matches our expectations, but that the number of quorum accesses actually decreases when we go from 10 to 15 writers. The reason is that at 15 writers, the effect of handling multiple snapshots together will manifest itself more clearly, since if a node invokes baseSnapshot() to help some other node, it would have invoked baseSnapshot() for itself anyway.



\OL{The old style of anticipation/result is below}

Lemma \ref{thm:latencyBounds} and \ref{thm:communicationCostsBounds} cannot be used to make a precise expectation of the snapshot latency for experiment 4, since there will be varying number of concurrent writers. But in general it is reasonable to expect that for fewer writers, the snapshot latency will be lower and closer to the lower bound. The same applies to the number of quorum accesses and reliable broadcasts.

The result of experiment 4 is shown in figures~\ref{fig:exp4_all} to~\ref{fig:exp4m_4}. We begin by looking at figure~\ref{fig:exp4_all}. There are several noteworthy observations. (1) The snapshot latency of algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} rapidly increases when the number of writers increase, and with 15 writers, most nodes could complete no snapshot operation at all during the five minutes the experiment was run for. This result illustrates that algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} indeed allow starvation of snapshotters. Note that with just one writer however, the snapshot latency is close to $\kappa$, which is what lemma \ref{thm:latencyBounds} anticipates. (2) Algorithm~\ref{alg:terminating} manages not to starve snapshotters and still be at least seven times faster than algorithm~\ref{alg:9disCongif}. This is due to Algorithm~\ref{alg:9disCongif} handling only one snapshot at a time, which we saw in section~\ref{sec:exp3}. The increase in latency, most visibly for Algorithm~\ref{alg:9disCongif}, is due to more interruptions and more work in the do-forever loop once the number of writers increses. Note that even for just one writer, the snapshot latency of Algorithm \ref{alg:9disCongif} is not close to the lower bound, which is because there are many snapshotters. (3) Algorithms~\ref{alg:9disCongif}, and~\ref{alg:terminating} for small values of $\delta$, do not starve writers, just as lemma \ref{thm:latencyBounds} states. More surprisingly, neither does Algorithm~\ref{alg:terminating} for $\delta = 1,000,000$. The reason for this is detailed in the next paragraph.

Figure~\ref{fig:exp4_4} shows the result of experiment 4 for just Algorithm~\ref{alg:terminating}. From this close-up we see that as the number of writers increases, the snapshot latency also increases but reaches a finite maximum. We also see that the snapshot latency for one writer is $\mu_2$, which lemma \ref{thm:latencyBounds} predicts. The increase is expected since when a node has to write, in addition to snapshot, its do-forever loop needs to handle one extra task. More writers also means all nodes' snapshots can be interrupted more often. We can also see that higher values of $\delta$ lead to slightly longer snapshot latencies. What is surprising is how similar the latencies are for different values of $\delta$, especially for higher number of writers, and that snapshotters are not starved for $\delta = 1,000,000$. This is due to the synchronization effect described in section~\ref{sec:exp2}.

Figure~\ref{fig:exp4m_all} shows the number of quorum accesses (related to snapshots) and reliable broadcast operations per snapshot operation for all algorithms. We see that as the number of writers increases, more and more quorum accesses are needed by algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}, since they become interrupted more often. For 15 writers they are starved and are performing quorum access all the time without getting anywhere. But for just a single writer, algorithms \ref{alg:0disCongif} and \ref{alg:disCongif} use few quorum accesses and are close to the lower bound of lemma \ref{thm:latencyBounds}. For Algorithm~\ref{alg:9disCongif}, the number of quorum accesses also increases when the number of writers increases, which is because they are interrupted more often. When the snapshots are interrupted more often, it takes a longer time to complete them, and more nodes get the chance to try to complete them, which will increase the number of reliable broadcasts. But the number of reliable broadcasts does not increase as fast as the number of quorum accesses, since there will be one extra reliable broadcast for each new node helping, but one extra quorum access for every interruption. The latter are more numerous.

From figure~\ref{fig:exp4m_all} we also see that the number of quorum accesses increases much faster for Algorithm~\ref{alg:9disCongif} compared to Algorithm~\ref{alg:terminating}. The reason is that when writers interrupt a snapshot operation, more quorum access are needed. But in Algorithm~\ref{alg:terminating}, since multiple snapshots are handled at the same time, the number of quorum accesses per snapshot operation will not grow as dramatically as for Algorithm~\ref{alg:9disCongif}. 

In figure~\ref{fig:exp4m_4} we see that the number of quorum accesses starts at slightly more than 2, one for the snapshot quorum access and one for $\sStore()$, which is also the lower bound of lemma \ref{thm:latencyBounds}. As the number of writers increases, more interruptions will happen and more snapshot quorum accesses are needed. But when the number of writers reaches 15, the effect of handling multiple snapshots at once will manifest itself more clearly. More writers means more interruptions and only after the first interruption, can another node help with the snapshot.

\subsubsection*{Experiment 5: The trade-off parameter $\delta$’s effect on write and snapshot latencies and number of messages sent}

\begin{figure}
\centering
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp5.pdf}
    \caption{The result of experiment 5. \newline \newline}
    \label{fig:exp5}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{snapshotEvaluation/exp5m.pdf}
    \caption{The result of experiment 5, showing number of quorum accesses per operation.}
    \label{fig:exp5m}
\end{minipage}
\end{figure}

From lemma \ref{thm:latencyBounds}, the lower bound on the write latency is $\mu_1$. We expect the write latency to converge towards this value as $\delta$ increases. From lemma \ref{thm:latencyBounds} we also know that the snapshot latency is unbounded for $\delta = infty$. We therefore expect the snapshot latency to increase dramatically when $\delta$ increases. From lemma \ref{thm:communicationCostsBounds} we know that the write operation will always use one quorum access. We also know that the snapshot operation will use at least two quorum accesses, but that it can grow unbounded when $\delta = \infty$. We therefore expect the number of quorum accesses to increase as $\delta$ increases.

Figure~\ref{fig:exp5} shows how the write and snapshot latencies change when the value of $\delta$ changes. The results show that the value of $\delta$ indeed plays a role for both operation latencies. Like expected, the write latency approaces $\mu_1$ and the snapshot latency rapidly increases, as $\delta$ increases. Note that the synchronization behavior described in section~\ref{sec:exp3} does not occur here since no node is both a writer and a snapshotter.

Figure~\ref{fig:exp5m} shows the number of quorum accesses needed per operation. We see that only one quorum access is needed for write operation, which matches the expectation. We also see that as $\delta$ increases, more quorum accesses are needed for the snapshot operation, which matches our expectation. It might seem surprising that higher values of $\delta$ lead to more snapshot-quorum accesses being performed, given we said that for $\delta > 0$, Algorithm~\ref{alg:terminating} aims at using only $O(n)$ messages. The reason is that the system is completely saturated with writes, so the nodes have no choice but to block the write operations to complete the snapshot operations. But for higher values of $\delta$, they wait longer, and do more quorum accesses while waiting. But since each node has to perform the snapshot eventually anyway, more quorum accesses are performed compared to just letting all nodes perform the snapshot immediately. In a real-usage scenario, it might be the case that there will be periods of $w$ writes and then a period without any writes. By setting $\delta = w$, we ensure that the snapshot operation will be patient enough to wait until the writes are done anyway, and then use $O(n)$ messages to complete. If for some reason the writes never stop, we still guarantee completion of all snapshot operations.

\subsection{Discussion}
    
%Explain how our observations answer each of our research questions. Explain what we cannot conclude from the experiments and requires further evaluation. Explain what was surprising. Explain which of our lessons could be useful also for other systems/evaluations/algorithms. 

Our first research question asks how well the system scales with respect to the number of writers and snapshotters. From the results, we see that the write latency and number of write-related quorum accesses of all algorithms, except Algorithm \ref{alg:terminating} for $\delta = 0$, remain largely unchanged when the number of writers and snapshotters increases. We also see that when there are no writers, the snapshot latency and number of snapshot-related quorum accesses of algorithms~\ref{alg:0disCongif},~\ref{alg:disCongif} and~\ref{alg:terminating} also remain largely unchanged when the number of snapshotters increases, while the snapshot latency of Algorithm~\ref{alg:9disCongif} increases linearly with the number of snapshotters. Finally, we also see that the snapshot latency and number of quorum accesses of algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} grow unbounded when the number of writers increases, but remain bounded and relatively unchanged for algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}. All in all, we see that algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif} scale well except when there are concurrent writes, that Algorithm~\ref{alg:9disCongif} does not starve snapshotters but does not scale well and that Algorithm~\ref{alg:terminating} scales well even with concurrent writes.

Our second research question asks what overhead we have to pay when comparing algorithms~\ref{alg:0disCongif} and~\ref{alg:disCongif}, as well as algorithms~\ref{alg:9disCongif} and~\ref{alg:terminating}. The results show that the overhead of algorithm~\ref{alg:disCongif} is very small compared to algorithm~\ref{alg:0disCongif}, in terms of latency and communication costs, for both write and snapshot operations. The results also show that Algorithm~\ref{alg:terminating} for $\delta = 0$ is at least as fast and communication cost-efficient as Algorithm~\ref{alg:9disCongif} in all tested scenarios, but also that Algorithm~\ref{alg:terminating} is much faster than Algorithm~\ref{alg:9disCongif} with respect to snapshot latency for large number of snapshotters.

Our third research question asks what role the trade-off parameter $\delta$ plays. The results show that $\delta$ indeed affects both the write latency and the snapshot latency. Increasing $\delta$ decreases the write latency, which converges to the smallest possible value, while the snapshot latency increases with increasing $\delta$.

What we cannot conclude is how the algorithms compare in terms of absolute performance. The thread-based implementation is not efficient and requires artifical delays, which means the system is no longer completely asynchronous. A more efficient implementation using an event-based approach could be an improvement. That way, no delays need to be used, which we clearly see have an effect on the latencies, and only the hardware and network would be the limitations. That an event-based implementation is likely more efficient is also the most important lesson we bring from this evaluation.

The most surprising discovery we made was the synchronization behavior of Algorithm~\ref{alg:terminating}, described in section~\ref{sec:exp2}. It is not obvious from the pseudocode that Algorithm~\ref{alg:terminating} with $\delta = \infty$ will behave close to $\delta = 0$. In a real-usage scenario this behavior has to be taken into account if a processor will be used for both write and snapshot operations from the client-side. This also means that we cannot conclude how the algorithms compare in non-synchronized scenarios.

} %remove that starts at section Results

